High Resolution Nonperturbative Light-Front Simulations of the True Muonium Atom

Through the development of a parallel code called TMSWIFT, an extensive light-front quantization study of the nonperturbative spectrum of the bound state $(\mu^+\mu^-)$, true muonium, has been performed. Using Pad\'{e} approximants, it has been possible to extract continuum and infinite-cutoff limits for the singlet and triplet states for a range of values of the coupling constant $\alpha$. This data set allows for an investigation of the $\alpha$ dependence of the light-front spectra, the results of which are compared to standard calculations. Decay constants have also been obtained. Improved calculations have been undertaken for the energy shifts due to the presence of a second, lighter flavor ($e$). Finally, initial results for three-flavor ($e$, $\mu$, $\tau$) calculations are presented.

==> Ealpha.tex <==
\begin{tabular}{l|c|c|c|c}
\hline\hline
$E_n$&$\alpha$&$M_0$&$N$&$\beta$\\ \hline
$1^1S_0$&[0.01,0.3]	&1.99988(5) & -0.392(13) &2.24(3)\\
        &[0.01,0.1]	&2.00000(1)&-0.28(2)& 2.04(3)\\
$1^3S_1$&[0.01,0.3]	&2.00002(2)& -0.2183(17)& 1.941(7)\\
        &[0.01,0.1]	&1.99999(1)& -0.248(16)& 2.01(3)\\
\hline
\end{tabular}

